Prompt Inference Attack on Distributed Large Language Model Inference Frameworks

The inference process of modern large language models (LLMs) demands prohibitive computational resources, rendering them infeasible for deployment on consumer-grade devices. To address this limitation, recent studies propose distributed LLM inference frameworks, which employ split learning principles to enable collaborative LLM inference on resource-constrained hardware. However, distributing LLM layers across participants requires the transmission of intermediate outputs, which may introduce privacy risks to the original input prompts - a critical issue that has yet to be thoroughly explored in the literature. In this paper, we rigorously examine the privacy vulnerabilities of distributed LLM inference frameworks by designing and evaluating three prompt inference attacks aimed at reconstructing input prompts from intermediate LLM outputs. These attacks are developed under various query and data constraints to reflect diverse real-world LLM service scenarios. Specifically, the first attack assumes an unlimited query budget and access to an auxiliary dataset sharing the same distribution as the target prompts. The second attack also leverages unlimited queries but uses an auxiliary dataset with a distribution differing from the target prompts. The third attack operates under the most restrictive scenario, with limited query budgets and no auxiliary dataset available. We evaluate these attacks on a range of LLMs, including state-of-the-art models such as Llama-3.2 and Phi-3.5, as well as widely-used models like GPT-2 and BERT for comparative analysis. Our experiments show that the first two attacks achieve reconstruction accuracies exceeding 90%, while the third achieves accuracies typically above 50%, even under stringent constraints. These findings highlight privacy risks in distributed LLM inference frameworks, issuing a strong alert on their deployment in real-world applications.

==> tex/ack.tex <==
\begin{acks}
To xxx
\end{acks}

==> tex/revisionletter.tex <==
\onecolumn
\thispagestyle{empty}
\centerline{\textbf{\Large Summary of Changes to CCS Submission $\#$467}}
\vspace{10mm}


\noindent We would like to thank all the reviewers and the Shepherd for their positive feedback and insightful comments.
%
In this letter, we present detailed responses to each revision criterion.
%
Changes in the revised paper are highlighted in {\color{blue} blue}.

% \vspace{2mm}\noindent
% \section*{Summary of Major Changes}
% \label{sec-changes}
% \vspace{2mm}\noindent
% We have made the following major changes in this revision:

% \begin{itemize}[topsep=2pt,itemsep=2mm,parsep=0pt,partopsep=0pt,leftmargin=20pt]
%     \item Section~\ref{sec-intro}: we have added more clarifications of technical challenges and the motivation of the threat model, in response to \textbf{revision criterion 1} and \textbf{2}.
%     \item Section~\ref{subsec-attack-1}: we have justified the Gaussian distribution assumption on Shapley values via a $\chi^2$ goodness-of-fit test, in response to \textbf{revision criterion 5}.
%     \item Section~\ref{subsec-attack-generalization}: we have added more discussion to clarify the technical novelty of our attacks, in response to \textbf{revision criterion 2}.
%     \item Section~\ref{sec-exp}: we have included additional experimental results with larger datasets, in response to \textbf{revision criterion 3}.
%     \item Section~\ref{sec-countermeasure}: we have discussed the countermeasure via mutual information and the countermeasure pointed by reviewer D, in response to \textbf{revision criterion 4} and \textbf{6}.
%     \item Section~\ref{sec-related-work}: we have added the discussion of the relation between Wang et al.'s work~\cite{wang2021privacy} and our attacks via mutual information, in response to \textbf{revision criterion 6}.
%     \item Section~\ref{sec-discussion}: we have added the discussion of the impact of large datasets on attack performance, in response to \textbf{revision criterion 3}.
% \end{itemize}

\vspace{2mm}\noindent
\section*{Response to Revision Criteria}

\vspace{2mm}\noindent
\textbf{Criterion 1.} \textit{Reframe the paper to focus on how privacy leaks instead of whether it leaks.}

\vspace{2mm}\noindent
\textbf{Response.} We have made three changes to reflect the reframing: 
\begin{itemize}
    \item In Section~\ref{sec-intro}, we revised the critical question from ``can intermediate outputs compromise the privacy of input
prompts?'' to ``to what extent can the privacy of input prompts be compromised via intermediate outputs?''.
    \item Still in Section~\ref{sec-intro}, we added the following clarification: ``While some developers of distributed LLM frameworks acknowledge potential
privacy risks associated with the transmission of intermediate results~\cite{Petals-acl}, they fail to provide definitive answers regarding \textit{how and
to what extent} private input prompts could be leaked''.
    \item In Section~\ref{subsec-dllmI}, we  similarly included: ``While some developers~\cite{Petals-acl} acknowledge potential privacy risks associated with sharing intermediate results, they fail to provide conclusive evidence or a comprehensive analysis of \textit{how and to what extent} input prompt privacy may be compromised''.
\end{itemize}


\vspace{2mm}\noindent
\textbf{Criterion 2.} \textit{Move discussion of defenses and limitations into the main text.}

\vspace{2mm}\noindent
\textbf{Response.} We have moved the discussion of defenses to Section~\ref{sec-defense} (\textit{Possible Countermeasures}), and the discussion of limitations to Section~\ref{sec-discussion}  (\textit{Discussion}).


\vspace{2mm}\noindent
\textbf{Criterion 3.} \textit{Expand the discussion of related work, as suggested by reviewer C.}

\vspace{2mm}\noindent
\textbf{Response.} As suggested by Reviewer C, we have thoroughly rewritten Section~\ref{sec-relatedwork} (\textit{Related Work}), removing the discussion on LLMs and expanding the analysis of embedding inversion attacks. The section structure has been revised from ``Large Language Models - Attacks on LLMs'' to ``Embedding Inversion Attacks - Other Types of Attacks''.


\vspace{2mm}\noindent
\textbf{Criterion 4.} \textit{Incorporate baselines ([ZMS24], [MKS+23]) and new metrics (cosine semantic similarity) as suggested by reviewers and discussed in rebuttal.}

\vspace{2mm}\noindent
\textbf{Response.} We have incorporated the baselines [ZMS24] (Output2Prompt~\cite{output2prompt}) and [MKS+23] (Vec2Text~\cite{MorrisKSR23promptinference}), as well as the new metric Cosine Semantic Similarity (CSS), into our experiments. The major changes include: 
\begin{itemize}
    \item Descriptions of CSS, Output2Prompt, and Vec2Text have been added to the Metric and Baselines sections in Section~\ref{sec-exp}.
    \item RA results comparing $\adv_1$ with Vec2Text have been added to Fig.~\ref{fig-attack1-accur}.
    \item RA and CSS results comparing $\adv_2$ with Vec2Text and Output2Prompt have been summarized in Table~\ref{tb-attack2-comp},  with reconstructed examples included in Table~\ref{tb-egg-adv2-in-paper}.
    \item CSS results for evaluating $\adv_3$ on Phi-3.5 and Llama-3.2 have been added to Table~\ref{tb-attack3-part2}.
    \item Additional discussions on the performance of $\adv_2$, Vec2Text, and Output2Prompt have been added to Section~\ref{subsec-exp-adv2}.
\end{itemize}


\vspace{2mm}\noindent


\section*{Response to Additional Comments in the Reviews}
\vspace{2mm}\noindent
\textbf{Review A - Comment 1.} \textit{The paper is missing details on the distributional differences in auxiliary data for Attack 2.}

\vspace{2mm}\noindent
\textbf{Response.} We have added further discussion on distributional differences for $\adv_2$ in Section~\ref{subsec-exp-adv2}: ``To better understand the relationship between $\adv_2$ performance and distributional differences between auxiliary and test datasets, we quantify the dataset distributional differences using Total Variation (TV) distance, which ranges from 0 (identical distributions) to 1 (no distribution overlap).
%
The TV between WikiText-2 and SQuAD2.0 is 0.4998, while the TV between WikiText-2 and Midjourney prompts is 0.7319, indicating that SQuAD2.0 shares greater distributional overlap with WikiText-2 compared to Midjourney prompts. This explains why $\adv_2$ trained on WikiText-2 consistently performs better on SQuAD2.0 than on Midjourney prompts''.


\vspace{2mm}\noindent
\textbf{Review A - Comment 2.} \textit{Does Attack 3 work on all models? I only see results for GPT2 and not Llama.}

\vspace{2mm}\noindent
\textbf{Response.} We have added  results for $\adv_3$ on Phi-3.5 and Llama-3.2 in Table~\ref{tb-attack3-part2}.

\vspace{2mm}\noindent
\textbf{Review A - Comment 3.} \textit{All chosen models have relatively few layers. What do you think the results would look like on LLMs with hundreds of layers?}

\vspace{2mm}\noindent
\textbf{Response.} We have added a discussion on \textit{Generalization to Deeper LLMs} in Section~\ref{sec-discussion}.


\vspace{5mm}\noindent
\textbf{Review B - Comment 1.} \textit{The defense evaluation of differential privacy in Appendix C is lacking important information. There is no metric reported for utility, and the strength of the defense is not varied.}

\vspace{2mm}\noindent
\textbf{Response.} We have conducted additional experiments by varying the privacy parameter and incorporating a utility metric.
The results are included in Table~\ref{tb-dp-defense-v2}, with the related discussion added to Section~\ref{sec-defense}.
Specifically, the privacy parameter $\eta$ (analogous to $\epsilon$ in traditional DP) is varied across $\{100, 500, \infty\}$ as in~\cite{defense-split-denoise}, where $\infty$ indicates no noise injection.
%
We use BERTScore (F1)~\cite{bertscore} to evaluate the LLM output utility under different levels of noise injection, where scores above 0.8 suggest strong semantic preservation, while scores below 0.7 indicate poor semantic output. 


\vspace{2mm}\noindent
\textbf{Review B - Comment 2.} \textit{Can you recover specific private information from prompts? A small benchmark of this would be convincing.}

\vspace{2mm}\noindent
\textbf{Response.} We have added a new private dataset, PrivatePrompts, in Section~\ref{sec-exp}, which
consists of 251,270 manually-crafted sensitive strings with inserted PII entities, such as name and date. Reconstruction performance and reconstructed examples tested on PrivatePrompts have been added to Table~\ref{tb-attack2-comp} and Table~\ref{tb-egg-adv2-in-paper}, respectively. Table~\ref{tb-egg-adv2-in-paper} shows that our attack can accurately reconstruct PII entities in PrivatePrompts.


\vspace{2mm}\noindent
\textbf{Review B - Comment 3.} \textit{Justify "these reconstruction methods are highly context-dependent, where an error in reconstructing a word can propagate and severely degrade the reconstruction accuracy for subsequent words".}

\vspace{2mm}\noindent
\textbf{Response.} We have added a footnote following the statement ``transformers reconstruct tokens sequentially, so errors in earlier tokens may negatively impact subsequent ones'' in Section~\ref{subsec-adv1} for justification. 


\vspace{2mm}\noindent
\textbf{Review B - Comment 4.} \textit{A simple baseline attack in this setting is to take the output layer of the model and apply it to every intermediate representation. How well does this work?}

\vspace{2mm}\noindent
\textbf{Response.} We have added a discussion on this baseline attack to Appendix~\ref{append-subsec-bll} (\textit{Linear Layer-based Baseline Attack}) in the full version of our paper~\cite{fullversion}.
%
We did not include it in the main text because this baseline assumes access to both the linear layer and intermediate embeddings, which is not consistent with the assumptions used in our attack evaluations.


\vspace{2mm}\noindent
\textbf{Review C - Comment 1.} \textit{Would a simple defense of the server first collecting multiple inputs, padding them, then querying them at the same time in a different order prevent the attack? Since now it would be hard to build the pairs of tokens and their embeddings that are used to train the classifiers.}

\vspace{2mm}\noindent
\textbf{Response.} We have added a discussion on the suggested defense, i.e., \textit{Shuffle the Prompts},
in Section~\ref{sec-defense} (\textit{Possible Countermeasures}).


\vspace{2mm}\noindent
\textbf{Review C - Comment 2.} \textit{The different PCA plots focus on very frequent stop words like 'the' and 'and'. Does this generalize to less frequent words? Also, does it generalize to tokens that are not complete words but depend on previous ones to be completed, e.g., 'ing'?}

\vspace{2mm}\noindent
\textbf{Response.} We have updated Fig.~\ref{fig-embd-scatter-adv1} by replacing tokens ` one' and ` which' with a less frequent word `ward' and a partial word `ing'. This modification does not affect our original observation of clustered embeddings.


\vspace{2mm}\noindent
\textbf{Review C - Comment 3.} \textit{Is there a reason why Llama and Phi are not included in the third scenario?}

\vspace{2mm}\noindent
\textbf{Response.} We have included $\adv_3$ results on Llama-3.2 and Phi-3.5 in Table~\ref{tb-attack3-part2}.



\vspace{2mm}\noindent
\textbf{Review C - Comment 4.} \textit{It would be interesting to see the limits of this attack in larger models.}

\vspace{2mm}\noindent
\textbf{Response.} Please refer to our response to \textbf{Review A - Comment 3} for discussion on \textit{Generalization to Deeper LLMs}.


\vspace{2mm}\noindent
\textbf{Review C - Comment 5.} \textit{In section 5.2, it is mentioned that the improvement is "(typically 30\%)"; however, looking at the plots, the jump is usually 20\%.}

\vspace{2mm}\noindent
\textbf{Response.} We have revised $30\%$ to $20\%$ in Section~\ref{subsec-exp-adv2}.


\vspace{2mm}\noindent
\textbf{Review C - Comment 6.} \textit{A very minor comment just out of curiosity: It would be interesting to see if the attack would work without any real data, so by only generating the synthetic dataset.}

\vspace{2mm}\noindent
\textbf{Response.} 
We did not incorporate the related discussion from the rebuttal into the revised paper, as the attack setting and insights from the initial results are similar to those of $\adv_3$.



\newpage
\twocolumn
